Learning Privately over Distributed Features: An ADMM Sharing Approach

Distributed machine learning has been widely studied in order to handle exploding amount of data. In this paper, we study an important yet less visited distributed learning problem where features are inherently distributed or vertically partitioned among multiple parties, and sharing of raw data or model parameters among parties is prohibited due to privacy concerns. We propose an ADMM sharing framework to approach risk minimization over distributed features, where each party only needs to share a single value for each sample in the training process, thus minimizing the data leakage risk. We establish convergence and iteration complexity results for the proposed parallel ADMM algorithm under non-convex loss. We further introduce a novel differentially private ADMM sharing algorithm and bound the privacy guarantee with carefully designed noise perturbation. The experiments based on a prototype system shows that the proposed ADMM algorithms converge efficiently in a robust fashion, demonstrating advantage over gradient based methods especially for data set with high dimensional feature spaces.

==> Makefile <==
#Makefile for LaTeX document files
# Created: July 3, 2015. Last modified: Feb 4, 2019.

# Set up the paths and names
# Default output is named "main". Default section path "./sections". Default figure path "./figures"
DOCUMENT=ms
SECPATH=sections/
FIGPATH=figures/

SECTIONS=$(wildcard $(SECPATH)*.tex)
FIGURES=$(wildcard $(FIGPATH)*.pdf)

$(DOCUMENT).pdf : $(DOCUMENT).tex $(SECTIONS) $(FIGURES) $(DOCUMENT).aux 
	pdflatex $(DOCUMENT).tex

$(FIGPATH)%.pdf : $(FIGPATH)%.eps 
	epstopdf $<

$(DOCUMENT).aux : $(DOCUMENT).bib
	latex $(DOCUMENT).tex
	bibtex $(DOCUMENT)
	latex $(DOCUMENT).tex
	latex $(DOCUMENT).tex

all : 
	latex $(DOCUMENT).tex
	bibtex $(DOCUMENT)
	latex $(DOCUMENT).tex
	latex $(DOCUMENT).tex
	pdflatex $(DOCUMENT).tex

clean:
	rm -rf *.aux $(DOCUMENT).log $(DOCUMENT).toc $(DOCUMENT).dvi \
    $(DOCUMENT).pdf $(DOCUMENT).bbl $(DOCUMENT).blg $(FIGPATH)*.pdf \
    $(DOCUMENT).out



==> sections/related.tex <==
\section{Related Works}

{\bf Differential Privacy Machine Learnings}\\
\cite{abadi2016deep} utilizes the momentum accountant method which yield a strong privacy bound. 

{\bf Distributed Machine Learning for Distributed Features}
\cite{heinze2017preserving} aims for linear based models, which projects and compress the original features and adds Gaussian noise to the projected features. Those features are distributed to other parties and each party train their own model with the provided features. (Information leakage is large. Need to justify this claim.)

{\bf DP+ADMM}
\cite{zhang2018improving} latest result for DP ADMM work. In this work, a modified version of ADMM where the penalty and the dual variable step size is decoupled as long as the penalty is increasing over the iterations and the penalty is greater than the dual variable step size. It is shown to converge in this modified ADMM. Further more, perturbation is applied on the penalty to guarantee the privacy. 

{\bf ADMM}

{\bf Important references}\\
\cite{huang2018dp} sublinear convergence rate. Due to linear approximation with a increasing strength for the quadratic term, convergence is guaranteed. Sensitivity is also decreasing. In the end, a decreased matching strength of noise is added. 

\cite{nishihara2015general} linear convergence rate. Strong assumption on the constraint matrix. One part should be invertible and the other part should be left-invertable. 

\cite{bellet2017personalized} Optimized noise budget. Not admm. 

\cite{shi2014linear}



{\bf Related works}\\
ADMM+DP\cite{zhang2016dual}


